Surrogate NAS Benchmarks: Going Beyond the Limited Search Spaces of Tabular NAS Benchmarks

The most significant barrier to the advancement of Neural Architecture Search (NAS) is its demand for large computational resources, which hinders scientifically sound empirical evaluations of NAS methods. Tabular NAS benchmarks have alleviated this problem substantially, making it possible to properly evaluate NAS methods in seconds on commodity machines. However, an unintended consequence of tabular NAS benchmarks has been a focus on extremely small architectural search spaces since their construction relies on exhaustive evaluations of the space. This leads to unrealistic results that do not transfer to larger spaces. To overcome this fundamental limitation, we propose a methodology to create cheap NAS surrogate benchmarks for arbitrary search spaces. We exemplify this approach by creating surrogate NAS benchmarks on the existing tabular NAS-Bench-101 and on two widely used NAS search spaces with up to $10^{21}$ architectures ($10^{13}$ times larger than any previous tabular NAS benchmark). We show that surrogate NAS benchmarks can model the true performance of architectures better than tabular benchmarks (at a small fraction of the cost), that they lead to faithful estimates of how well different NAS methods work on the original non-surrogate benchmark, and that they can generate new scientific insight. We open-source all our code and believe that surrogate NAS benchmarks are an indispensable tool to extend scientifically sound work on NAS to large and exciting search spaces.

==> sections/10_reproducibility.tex <==
\section{Reproducibility Statement}\label{app:nas_checklist}

% ICLR 2022: Authors are strongly encouraged to include a paragraph-long Reproducibility Statement at the end of the main text (before references) to discuss the efforts that have been made to ensure reproducibility. This paragraph should not itself describe details needed for reproducing the results, but rather reference the parts of the main paper, appendix, and supplemental materials that will help with reproducibility. 

For our reproducibility statement, we use the ``NAS Best Practices Checklist'' \citep{best_practices}, which was recently released to improve reproducibility in neural architecture search.

%In the past, the field of NAS research has had problems with reproducibility and fairness in experimental comparisons~\citep{randomnas, nasbench, yang2019evaluation}. A NAS best practices checklist was recently released~\citep{lindauer2019best}, and we address each question below.


\begin{enumerate}

\item \textbf{Best Practices for Releasing Code}\\[0.2cm]
For all experiments you report: 
\begin{enumerate}
  \item Did you release code for the training pipeline used to evaluate the final architectures?
    \answerYes{Follow link in the footnote of page 2 (Section~\ref{sec: introduction}). The training pipeline and hyperparameters used to train the architectures are clearly specified in the corresponding scripts.}
  \item Did you release code for the search space
    \answerYes{The used search spaces are the ones from DARTS~\citep{darts} and FBNet~\citep{fbnet}.}
\item Did you release the hyperparameters used for the final evaluation pipeline, as well as random seeds?
  \answerYes{Follow link in the footnote of page 2 (Section~\ref{sec: introduction}). We released our code, which includes the seeds and final evaluation pipeline used. The hyperparameters for training the architectures are fixed, while the ones for training the surrogate models are optimized using BOHB~\citep{Falkner18}.}
  \item Did you release code for your NAS method?
  \answerYes{All of our code for benchmarking NAS methods is available by following the same link to the codebase.}
  %\url{https://github.com/automl/naslib}.}
  \item Did you release hyperparameters for your NAS method, as well as random seeds?
  \answerYes{The hyperparameters we used are also available.}   
\end{enumerate}

\item \textbf{Best practices for comparing NAS methods}
\begin{enumerate}
  \item For all NAS methods you compare, did you use exactly the same NAS benchmark, including the same dataset (with the same training-test split), search space and code for training the architectures and hyperparameters for that code?
    \answerYes{Refer to Section~\ref{sec:methods} for details.}
  \item Did you control for confounding factors (different hardware, versions of DL libraries, different runtimes for the different methods)?
    \answerYes{We trained all the architectures on the same GPU (Nvidia RTX2080 Ti) and used the same versions of the used libraries to run all NAS methods.}	
    \item Did you run ablation studies?
    \answerYes{We show ablation studies in Section \ref{subsec:loo_analysis}.}
	\item Did you use the same evaluation protocol for the methods being compared?
    \answerYes{}
	\item Did you compare performance over time?
    \answerYes{We typically compare the anytime performance of black-box NAS optimizers for a specified time budget. See the figures in Section~\ref{sec:methods} for examples.}
	\item Did you compare to random search?
    \answerYes{We did include random search in our experiments in Section \ref{sec:methods} and data collection.}
	\item Did you perform multiple runs of your experiments and report seeds?
    \answerYes{We run the black-box optimizers on the surrogate benchmark multiple times and average the results.}
	\item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    \answerYes{This is in fact the main purpose of our paper: to introduce realistic surrogate NAS benchmarks.}

\end{enumerate}

\item \textbf{Best practices for reporting important details}
\begin{enumerate}
  \item Did you report how you tuned hyperparameters, and what time and resources
this required?
    \answerYes{We reported this information in Section~\ref{subsec:eval_data_fit}.}
  \item Did you report the time for the entire end-to-end NAS method
    (rather than, e.g., only for the search phase)?
    \answerYes{Our results use the end-to-end time.}
  \item Did you report all the details of your experimental setup?
    \answerYes{We did include all details of the setup in Section \ref{sec:methods}.}

\end{enumerate}
\end{enumerate}


==> sections/111_improving_surrogates.tex <==
\section{Improving Data Fit for Good Architectures}
\label{sec:improving_data_fit}

Since some search spaces, such as the DARTS one (detailed description in Appendix~\ref{subsec:background:search_space}), are far too large to be exhaustively evaluated, care has to be taken when sampling the architectures which will be used to train the surrogate models. As we showed in the previous section, surrogate models can effectively interpolate in the space when fitted on random data only. However, in most of the cases we design NAS algorithms with the hope that they will tend to exploit well-performing regions of the space efficiently. Therefore, when creating surrogate benchmarks we sometimes care more that the surrogate model will provide better predictive performance on these well-performing regions. Below, we propose a general methodological extension that can be used to improve the surrogate model by using well-performing architectures sampled from various NAS optimizers, without overfitting on a particular one.
%Sampling should yield a good overall coverage of the architecture space while also providing a special focus on the well-performing regions that optimizers tend to exploit.

Our principal methodology is inspired by~\cite{eggensperger-aaai15}, who collected unbiased data about hyperparameter spaces by random search (RS), as well as biased and dense samples in high-performance regions by running hyperparameter optimizers. 
%This is desirable for a surrogate benchmark since we are interested in evaluating NAS methods that exploit such good regions of the space. 
Table~\ref{tab:results:optimizer_configs} in the appendix lists the NAS methods we used to collect such samples and the respective number of samples. Additionally, we evaluated $\sim$1k architectures in poorly-performing regions for better coverage and another $\sim$10k for the analysis conducted on the dataset and surrogates. We refer to Appendices~\ref{subsec:app:data_collection} and \ref{sec:details_optimizers} for details on the data collection and the optimizers, respectively. 
%We would like to point out that in hindsight adding training data of well-performing regions may be less important for a surrogate NAS benchmark than for a surrogate HPO benchmark, which we demonstrated in Appendix~\ref{subsec:only_rs}. We believe that this is a result of HPO search spaces containing many configurations that yield dysfunctional models, which is less common for architectures in many NAS search spaces, hence allowing random search to provide a good coverage of the space.

In Figure~\ref{fig:exp:data_statistics:tsne:val_accuracy} in the appendix, we visualize the overall coverage of the search space, as well as the similarity between sampled architectures using t-SNE~\citep{maaten2008visualizing}. Besides showing a good overall coverage, some well-performing architectures in the search space form distinct clusters which are mostly located outside the main cloud of points. This clearly indicates that architectures with similar performance are close to each other in the architecture space. We also observe that different optimizers sample different architectures (see Figure~\ref{fig:exp:data_statistics:tsne_algo_comparison} in the appendix).

\subsection{Leave One-Optimizer-Out Analysis}
\label{subsec:loo_analysis}

Since the aim of a surrogate benchmark is to allow efficient benchmarking of novel NAS algorithms, it is necessary to ensure that the surrogate model can deliver accurate performance estimation on data from trajectories by unseen NAS methods. Similarly to \cite{eggensperger-aaai15}, we therefore perform a form of cross-validation on the optimizers we used for data collection, i.e., we leave out all data collected by one of the NAS methods entirely during training (using a stratified 0.9/0.1 train/val split over the other NAS methods). Then, we predict the unseen results from the left-out NAS method to evaluate how well the models extrapolate to the region covered by the `unseen' method. We refer to this as the leave-one-optimizer-out (LOOO) setting. 

\begin{figure}[t]
    \centering
    \includegraphics[width=.97\textwidth]{figures/results/trajectories/loo/benchmark_looo-min.jpg}
    %\vspace{-8mm}
    \caption{Anytime performance of blackbox optimizers, comparing performance achieved on the real benchmark and on surrogate benchmarks built with GIN and XGB in an LOOO fashion. 
    %\noteaz{Do I look this wrong, or does actually adding data from optimizers make things worse compared to Fig 2?\\FH: hmm, indeed, this does not make a strong case for adding data from optimizers. How does it look when we use all the data (not LOOO)?\\ AZ: That would be Fig. 23}
    }
    \label{fig:blackbox_trajectory_loo}
\end{figure}

\vspace{-3mm}
\paragraph{Results.}
%The results in Table~\ref{tab:looo_regression} show that the rank correlation between the predicted and observed validation accuracy remains high even when a well-performing optimizer such as RE is left out. Predicting BANANAS in the LOOO fashion yields a lower rank correlation, because it focuses on well-performing architectures that are harder to rank; however, the high $R^2$ shows that the fit is still good. 

%Conversely, leaving out DARTS causes a low $R^2$ but still high sKT; this is due to architectures with many skip connections in the DARTS data that are overpredicted (further discussed in Section~\ref{subsec:oneshot_trajectories}).
%For full details, Figure~\ref{fig:exp:data_statistics:leave_one_optimizer_out_analysis} in the appendix provides scatter plots of the predicted vs. true performance for each NAS method.

Figure~\ref{fig:blackbox_trajectory_loo} shows the trajectories in the leave-one-optimizer-out setting. The $\texttt{SNB-DARTS-XGB}$ and $\texttt{SNB-DARTS-GIN}$ surrogates again capture the general behavior of different optimizers well, illustrating that characteristics of new optimization algorithms can be captured with the surrogate benchmark. Leaving out DE appears to be a bigger problem for XGB than GIN, pointing to advantages of the smooth embedding learned by the GIN compared to gradient-boosting.
    
In an additional experiment, we found that surrogates built on only well-performing architectures (92\% and above) yielded poor extrapolation to worse architectures, but that surrogate benchmarks based on them still yielded realistic trajectories. We attribute this to NAS optimizers' focus on good architectures. For details, see Appendix~\ref{subsubsec:ablation_study}. 
%We also investigate whether it is possible to create benchmarks only on random architectures in Appendix~\ref{subsec:only_rs}, and find that we can indeed obtain realistic trajectories but lose some predictive performance in the well-performing regions. 
%Nevertheless, such benchmarks have the advantage of not possibly favouring any NAS optimizer used for the generation of training data, and we thus recommend their release in addition to the benchmarks based on the full training data.

% \begin{figure}
%     \centering
%     \includegraphics[width=.95\textwidth]{figures/results/trajectories/all_data/benchmark_all_data.jpg}
%     %\vspace{-8mm}
%     \caption{Anytime performance of different optimizers on the real benchmark (left) and the surrogate benchmark (GIN (middle) and XGB (right)) when training ensembles on data collected from all optimizers. Trajectories on the surrogate benchmark are averaged over 5 optimizer runs and the standard deviation is depicted.}
%     \label{fig:blackbox_trajectory}
% \end{figure}



==> sections/111_results.tex <==
%\section{Results for the First Surrogate Benchmarks}
\section{Surrogate Benchmarks for Evaluating NAS Optimizers}
\label{sec:results}

Having assessed the ability of the surrogate models to fit the search space, we now evaluate the surrogate NAS benchmarks $\texttt{SNB-DARTS-XGB}$ and $\texttt{SNB-DARTS-GIN}$, comparing cheap evaluations of various NAS algorithms on them against their expensive counterpart on the original non-tabular NAS benchmarks.
%
We note that for the surrogate trajectories, each architecture evaluation is sampled from the surrogate model's predictive distribution for the given architecture. Therefore, different optimizer runs lead to different trajectories.
    
\subsection{Evaluating the NAS surrogate benchmarks $\texttt{SNB-DARTS-XGB}$ and $\texttt{SNB-DARTS-GIN}$}
\label{subsec:blackbox_trajectories}
    
\begin{figure}
    \centering
    \includegraphics[width=.9\textwidth]{figures/results/trajectories/all_data/benchmark_all_data.jpg}
    %\vspace{-8mm}
    \caption{Anytime performance of different optimizers on the real benchmark (left) and the surrogate benchmark (GIN (middle) and XGB (right)) when training ensembles on data collected from all optimizers. Trajectories on the surrogate benchmark are averaged over 5 optimizer runs and the standard deviation is depicted.}
    \label{fig:blackbox_trajectory}
\end{figure}
    
We first compare the trajectories on the true, original, non-tabular benchmark and on the surrogate benchmarks for blackbox optimizers when training the surrogate on all data. For the true benchmark, we show the trajectories we ran to create our dataset (based on a single run per optimizer, since we could not afford repetitions due to the extreme compute requirements of 115 GPU days for a single run). For the evaluations on the surrogate, on the other hand, we can trivially afford to perform multiple runs. 

\vspace{-3mm}
\paragraph{Results (all data).}
As Figure~\ref{fig:blackbox_trajectory} shows, both the XGB and the GIN surrogate capture behaviors present in the true benchmark. For instance, the strong improvements of BANANAS and RE are also present on the surrogate benchmark at the correct time. In general, the ranking of the optimizers towards convergence is accurately reflected on the surrogate benchmark. Also, the initial random exploration of algorithms like TPE, RE and DE is captured as the large initial variation in performance indicates. Notably, the XGB surrogate ensemble exhibits a high variation in well-performing regions as well and seems to slightly underestimate the error of the best architectures. The GIN surrogate, on the other hand, shows less variance in these regions but slightly overpredicts for the best architectures.
    
Note, that due to the size of the search space, random search stagnates and cannot identify one of the best architectures even after tens of thousands of evaluations, with BANANAS finding better architectures orders of magnitude faster. This is correctly reflected in both surrogate benchmarks.
%This stands in contrast to previous NAS benchmarks. For instance, NAS-Bench-201~\citep{dong20} only contains 6466 unique architectures in total, causing the median of random search runs to find the best architecture after only 3233 evaluations.
    
\begin{figure}
    \centering
    \includegraphics[width=.9\textwidth]{figures/results/trajectories/loo/benchmark_looo-min.jpg}
    \vspace{-1.9mm}
    \caption{Anytime performance of blackbox optimizers, comparing performance achieved on the real benchmark and on surrogate benchmarks built with GIN and XGB in an LOOO fashion.
    \vspace{-2mm}
    }
    \label{fig:blackbox_trajectory_loo}
\end{figure}
    
To simulate benchmarking of novel NAS methods, we expand on the leave-one-optimizer-out analysis (LOOO) from Section~\ref{subsec:loo_analysis} and assess each optimizer with surrogate benchmarks based on data excluding that gathered by said optimizer. We again compare the trajectories obtained from 5 runs on the surrogate benchmark to the groundtruth.
    
\vspace{-3mm}
\paragraph{Results (LOOO).} Figure~\ref{fig:blackbox_trajectory_loo} shows the trajectories in the leave-one-optimizer-out setting. The XGB and GIN surrogates again capture the general behavior of different optimizers well, illustrating that characteristics of new optimization algorithms can be captured with the surrogate benchmark. Leaving out DE appears to be a bigger problem for XGB than GIN, pointing to advantages of the smooth embedding learned by the GIN compared to gradient-boosting.
    
In an additional experiment, we found that surrogates built on only well-performing architectures (92\% and above) yielded poor extrapolation to worse architectures, but that surrogate benchmarks based on them still yielded realistic trajectories. We attribute this to NAS optimizers' focus on good architectures. For details, see Appendix~\ref{subsubsec:ablation_study}. We also investigate whether it is possible to create benchmarks only on random architectures, and find that we can indeed obtain realistic trajectories (see Figure~\ref{fig:trajectories_only_rs} in the appendix) but lose some predictive performance in the well-performing regions. For the full description of this experiment see Appendix~\ref{subsec:only_rs}. Nevertheless, such benchmarks have the advantage of not possibly favouring any NAS optimizer used for the generation of training data, and we thus recommend their release in addition to the benchmarks based on the full training data.

%\begin{figure}[ht]
%    \centering
%    \vspace{-3mm}
%    \includegraphics[width=.97\textwidth]{figures/results/trajectories/ablation/benchmark_all_data_only_rs.png}
%    %\vspace{-4mm}
%    \caption{Anytime performance of different optimizers on the real benchmark (left) and the surrogate benchmark (GIN (middle) and XGB (right)) when training ensembles only on data collected by random search. Trajectories on the surrogate benchmark are averaged over 5 optimizer runs.}
%    \label{fig:trajectories_only_rs}
%\end{figure}


Finally, surrogate NAS benchmarks
%, like $\texttt{SNB-DARTS-GIN}$ and $\texttt{SNB-DARTS-XGB}$, 
can also be used to monitor the behavior of one-shot NAS optimizers throughout their search phase, by querying the surrogate model with the currently most promising discrete architecture. We show this evaluation in Appendix~\ref{subsubsec:one_shot_full}.

%\notefh{Arber, please move the text below to the appendix}
    
% \subsection{One-shot Optimizers}
% \label{subsec:oneshot_trajectories}
    
% %\noteaz{Decide based on space if we will keep this.}

% Surrogate NAS benchmarks, like NAS-Bench-301, can also be used to monitor the behavior of one-shot NAS optimizers throughout their search phase, by querying the surrogate model with the currently most promising discrete architecture. This can be extremely useful in many scenarios since uncorrelated proxy (performance of the one-shot model) and true objectives (performance of the fully trained discretized architecture) can lead to potential failure modes, e.g., to a case where the found architectures contain only skip connections in the normal cell~\citep{zela19, zela2020nasbenchshot, dong20} (we study such a failure case in Appendix~\ref{subsubsec:one_shot_full} to ensure robustness of the surrogates in said case). We demonstrate this use case in a similar LOOO analysis as for the black-box optimizers, using evaluations of the discrete architectures from each search epoch of multiple runs of DARTS, PC-DARTS and GDAS as ground-truth. Figure~\ref{fig:oneshot_trajectory_loo} shows that the surrogate trajectories closely resemble the true trajectories.

\subsection{Evaluating the NAS surrogate benchmark $\texttt{SNB-FBNet-XGB}$}
\label{subsec:blackbox_trajectories_fbnet}

\begin{figure}
    \centering
    \includegraphics[width=.49\textwidth]{figures/fbnet/True.pdf}
    \includegraphics[width=.49\textwidth]{figures/fbnet/Surr.pdf}
    %\vspace{-8mm}
    \caption{Anytime performance of different optimizers on the real benchmark and the XGB surrogate benchmark when training ensembles on data collected only from random search. Trajectories on the surrogate benchmark are averaged over 5 optimizer runs and the standard error is depicted.}
    \label{fig:blackbox_trajectory}
\end{figure}

    

==> sections/7_limitation.tex <==
\section{Societal Impact, Limitations \& Guidelines for Using Surrogate Benchmarks}
\label{sec:limitations}

We hope and expect that the NAS practitioner will benefit from our \emph{surrogate} NAS benchmarks the same way for research on exciting large search spaces as she so far benefited from \emph{tabular} NAS benchmarks for research on toy search spaces -- by using them for fast and easy prototyping of algorithms and large-scale (yet cheap) scientific evaluations. We expect that in the next years this will save millions of GPU hours (which will otherwise be spent on running expensive NAS benchmarks) and thus help reduce the potentially hefty carbon emissions of NAS research~\cite{Hao19}. It will also ensure that the entire NAS community can partake in exploring large and exciting NAS design spaces, rather than only corporations with enormous compute power, thereby further democratizing NAS research.
%We also believe that our detailed guidelines on how to build surrogate benchmarks will lead to the creation of more interesting benchmarks with much larger and complex search spaces, different from the ones that the NAS community has been overfitting so far.

%We hope that surrogate NAS benchmarks in general will allow the NAS practitioner to quickly prototype and benchmark NAS algorithms without requiring large computational resources, and that \mbox{NAS-Bench-301} in particular will allow doing so on the currently most widely used search space. 

%However, we would also like to point out a risk of surrogate NAS benchmarks and how to guard against it. 
However, we would like to point out that there exists a risk that prior knowledge about the surrogate model used in a particular benchmark could lead to the design of algorithms that overfit that benchmark. To this end, we recommend the following best practices to ensure a safe and fair benchmarking of NAS methods on surrogate NAS benchmarks:

\vspace*{-0.06cm}
\begin{itemize}[leftmargin=*]
    \item The surrogate model should be treated as a black-box function, hence only be used for performance prediction and not exploited to extract, e.g., gradient information.
    \item We discourage benchmarking methods that internally use the same model as the surrogate model picked in the surrogate benchmark (e.g. GNN-based Bayesian optimization should not only be benchmarked using a GIN surrogate benchmark).
    \item We encourage running experiments on versions of surrogate benchmarks that are based on (1) all available training architectures and (2) only architectures collected with uninformed methods, such as random search or space-filling designs. As shown in Appendix~\ref{subsec:only_rs}, (1) yields better predictive models, but (2) avoids any potential bias (in the sense of making more accurate predictions for architectures explored by a particular type of NAS optimizer) and can still yield strong benchmarks. 
    \item In order to ensure comparability of results in different published papers, we ask users to state the benchmark's version number. So far, we release $\texttt{SNB-DARTS-XGB-v1.0}$, $\texttt{SNB-DARTS-GIN-v1.0}$, $\texttt{SNB-DARTS-XGB-rand-v1.0}$, and $\texttt{SNB-DARTS-GIN-rand-v1.0}$.
\end{itemize}
\vspace*{-0.06cm}

Due to the flexibility of surrogate NAS benchmarks to tackle arbitrary search spaces, we expect that the community will create many such benchmarks in the future, just like it already created many tabular NAS benchmarks~\cite{ying19a,dong20,zela2020nasbenchshot,dong2020nats,klein2019tabular,klyuchnikov2020bench,mehrotra2021nasbenchasr,li2021hwnasbench}.
%(and in fact even more so, since the limitation to search spaces that could be evaluated exhaustively does not apply to surrogate NAS benchmarks). 
We therefore collect best practices for the creation of such new surrogate NAS benchmarks in Appendix \ref{sec:guidelines_for_creating_surr_benches}. 
